Class of Trustworthy Pseudo-Random Number Generators

With the widespread use of communication technologies, cryptosystems are therefore critical to guarantee security over open networks as the Internet. Pseudo-random number generators (PRNGs) are fundamental in cryptosystems and information hiding schemes. One of the existing chaos-based PRNGs is using chaotic iterations schemes. In prior literature, the iterate function is just the vectorial boolean negation. In this paper, we propose a method using Graph with strongly connected components as a selection criterion for chaotic iterate function. In order to face the challenge of using the proposed chaotic iterate functions in PRNG, these PRNGs are subjected to a statistical battery of tests, which is the well-known NIST in the area of cryptography.

==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> generalizingPRNGAlgorithm.tex <==

\subsection{Old CI PRNG}
This sections present a generalisation of the previous algorithm 
leading to a scheme of PRNG. 


First of all, the double use of the  \textit{XORschift} algorithm was guided by 
experiments. In what follows, we consider the algorithm to 
be parameterized by any pair $(r_1,r_2)$ of pseudo randon number generators.


Finally, the negation function may be replaced by any function $f$ 
whose iterations have been proven to be chaotic. 



%\begin{figure}
\begin{algorithm}
\SetAlgoLined
%\SetLine
\KwData{$r_1$, $r_2$ generators, $f$ and $g$ function} 
\KwIn{the internal configuration $x$ ($n$ bits)}
\KwOut{a configuration $r$ ($n$ bits)}
$m\leftarrow{g(r_1(),x,f)}$\;
\For{$i=0,\dots,m$}
{
$S\leftarrow{r_2() \mod n} $\;
$x_S\leftarrow{f_S(x)}$\;
}
$r\leftarrow{x}$\;
return $r$\;
\medskip
\caption{Pseudo Random Number Generator}
\label{algo:old}
\end{algorithm}



Parameters $r_1$, $r_2$, $f$ and $g$ are defined as follows: 
\begin{itemize}
\item $r_1$ and $r_2$ are two pseudo random number generators 
that follow a discrete uniform distribution on
$\llbracket 0, 2^n-1\rrbracket$; 
\item $f = (f_1,\ldots,f_n) \in \Bool^n \rightarrow \Bool^n$  is 
  a function that modifies the value of the internal vector $x$.
  We constrain $f$ to have a strongly connected iteration graph $\Gamma(f)$.
  Let then $n_x$ be the lenght of the longest path from $x$ to any 
  other configuration in $\Gamma(f)$.
\item for a given function $f$ and a given configuration $x$, 
the function $g$ has the following signature: 
$g: \llbracket 0, 2^n-1 \rrbracket \rightarrow 
\llbracket 0, n_x\rrbracket$ .
It transforms a number $k$ from
a uniforms distribution on $\llbracket 0,  2^n-1 \rrbracket$
into a number $m$ with such a  property: 
the size of the configuration set that may be reached from $x$ 
following a path of length $m$ (without cycle) is 
proportionnal to the frequency of $m$ in the distribution on
$\llbracket 0, n_x\rrbracket$. 
\end{itemize}

Let us first show how the Algorithm presented in~\cite{bgw09:ip}
is an instance of this scheme.

Obviously  $r_1$ and $r_2$ are the \textit{XORshift} PRNG.
$f$ is the vectorial boolean negation (\textit{i.e} 
$f(x_1,\ldots,x_n)=(\overline{x_1},\ldots,\overline{x_n})$).
In this context, since there is a arc  $(x,y)$ from any configuration 
$x$ to any neighbor $y$ of $x$, the length of the longest path from $x$ 
to any other configuration $z$ is $n$. 
We first deduce that $n_x$ is constantly equal to  $n$ and  
that $g$ does not depend on $x$. 
For a given input configuration $x \in \Bool^n$ , the algorithm 
outputs a new configuration  $r$ in $\Bool^n$ 
  





Let $n \in \Nats^*, n \geqslant 2$. Some chaotic iterations are fulfilled to generate a sequence $\left(x^t\right)_{n\in\Nats} \in \left(\Bool^n\right)^\Nats$ of boolean vectors: the successive states of the iterated system. Some of these vectors are randomly extracted and their components constitute our pseudorandom bit flow.

Chaotic iterations are realized as follows. Initial state $x^0 \in \Bool^n$ is a boolean vector taken as a seed and chaotic strategy $\left(S^t\right)_{n\in\Nats}\in \llbracket 1, n \rrbracket^\Nats$ is constructed with PRNG2. Lastly, iterate function $f$ is the vectorial boolean negation
$$f_0:(x_1,...,x_n) \in \Bool^n \longmapsto (\overline{x_1},...,\overline{x_n}) \in \Bool^n.$$
To sum up, at each iteration only $S^i$-th component of state $X^t$ is updated, as follows
\begin{equation}
x_i^t = \left\{\begin{array}{ll}x_i^{t-1} & \text{if } i \neq S^i, \\ \\ \overline{x_i^{t-1}} & \text{if } i = S^i. \\\end{array}\right.
\end{equation}
Finally, let $\mathcal{M}$ be a finite subset of $\Nats^*$. Some $x^t$ are selected by a sequence $m^t$ as the pseudorandom bit sequence of our generator. The sequence $(m^t)_{n \in \Nats} \in \mathcal{M}^\Nats$ is computed with PRNG1. So, the generator returns the following values: the components of $x^{m^0}$, followed by the components of $x^{m^0+m^1}$, followed by the components of $x^{m^0+m^1+m^2}$, \emph{etc.}
In other words, the generator returns the following bits:

\begin{small}
\noindent $x_1^{m_0}x_2^{m_0}x_3^{m_0}\hdots x_n^{m_0}x_1^{m_0+m_1}x_2^{m_0+m_1}x_3^{m_0+m_1}\hdots x_n^{m_0+m_1}$
$x_1^{m_0+m_1+m_2}x_2^{m_0+m_1+m_2}x_3^{m_0+m_1+m_2}...$
\end{small}
%and its $k^{th}$ bit is equal to $$\displaystyle{x_{k+1 \text{ (mod }n\text{)}}^{\sum_{i=0}^{\lfloor k/n \rfloor}m_i}}.$$

\noindent or the following integers:$$x^{m_0}x^{m_0+m_1}x^{m_0+m_1+m_2}\hdots$$

The basic design procedure of the novel generator is summed up in Table~\ref{Chaotic iteration}.
The internal state is $x$, the output array is $r$. $a$ and $b$ are those computed by PRNG1 and PRNG2. Lastly, $k$ and $n$ are constants and \linebreak $\mathcal{M}=\{$k, k+1$\}$ ($k\geqslant 3n$ is recommended).



\subsection{Mapping function}

\begin{definition}
The set $\Bool$ denoting $\{0,1\}$, let $f:\Bool^{n%
}\longrightarrow \Bool^{n}$ be an ``iteration'' function. Then, the mapping function $F$ is defined by
$F=(f(0),f(1),\ldots,f(2^{n}))$
\end{definition}

For example, if $n=3$ and iterate function $f$ is the vectorial boolean negation
$f_0:(x_1,x_2,x_3) \in \Bool^3 \longmapsto (\overline{x_1},\overline{x_2},\overline{x_3}) \in \Bool^3$ as following Table~\ref{F}, then
$F=(7,6,5,4,3,2,1,0)$
\begin{table}

\caption{Example of successive substitutions}
\label{F}
\centering
  \begin{tabular}{cccc}
    \hline
State 	& $\Bool^3$& $f$ 	&State   \\ \hline
0	&0,0,0		&1,1,1	&7\\
1	&0,0,1		&1,1,0	&6\\
2	&0,1,0		&1,0,1	&5\\
3	&0,1,1		&1,0,0	&4\\
4	&1,0,0		&0,1,1	&3\\
5	&1,0,1		&0,1,0	&2\\
6	&1,1,0		&0,0,1	&1\\
7	&1,1,1		&0,0,0	&0\\
    \hline
  \end{tabular}
\end{table}

\subsection{CI algorithm}
The basic design procedure of the CI generator with various functions is shown in Algorithm~\ref{CI Algorithm}.

\begin{algorithm}
\KwIn{afunction $f$, an iteration number $b$, an initial state $x^0$ ($n$ bits)}
\KwOut{a state $x$ ($n$ bits)}
$x\leftarrow x^0$\;
$k\leftarrow b + (\textit{XORshift}() \mod 2)}$\;
\For{$i=0,\dots,k-1$}
{
$s\leftarrow{\textit{XORshift}() \mod n}$\;
$x\leftarrow{F_f(s,x)}$\;
}
return $x$\;
\medskip
\caption{An arbitrary round of the CI PRNG with various functions}
\label{CI Algorithm}
\end{algorithm}


\subsection{Illustrative Example}

In this example, $n = 4$ and $\mathcal{M} = \{$4,5$\}$ are chosen for easy understanding.
The initial state of the system $x^0$ can be seeded by the decimal part of the current time. For example, the current time in seconds since the Epoch is 1237632934.484088, so $t = 484088$. $x^0 = t \text{ (mod 16)}$ in binary digits, then $x^0 = (0, 1, 0, 0)$. $m$ and $S$ can now be computed from PRNG1 and PRNG2:
\begin{itemize}
\item $F$ = (14, 14, 12, 12, 10, 10, 9, 9, 6, 6, 4, 4, 2, 2, 1, 0)
\item $m$ = 4, 5, 4, 4, 4, 4, 5, 5, 5, 5, 4, 5, 4,...
\item $S$ = 2, 4, 2, 3, 4, 1, 1, 4, 4, 3, 2, 3, 3,...
\end{itemize}
Chaotic iterations are done with initial state $x^0$, the mapping function $F$, and strategy $S$. The result is presented in Table \ref{table application example}. Let us recall that sequence $m$ gives the states $x^t$ to return: $x^4, x^{4+5}, x^{4+5+4}, \hdots$\newline
\begin{tiny}
\begin{table*}[!t]
%\renewcommand{\arraystretch}{1.3}
\centering
\begin{tabular}{|c|ccccc|cccccc|cccccc|}
\hline\hline
$m:$ & & & 4 & & & & & 5 & & & & & & 4 & & & \\ \hline
$S$ & 2 & 4 & 2 & 3 & & 4 & 1 & 1 & 4 & 4 & & 3 & 2 & 3 & 3 & & \\ \hline
 &$F^4$&$F^0$&$F^0$&$F^4$ &  &$F^6$ &$F^7$ &$F^{15}$ &$F^7$ &$F^7$ & &$F^7$ &$F^5$ & $F^1$& $F^3$&  & \\
%1ere ligne
 & 1& 1& 1& 1&
 & 1& \textbf{1} & \textbf{0} &1 &1 &
 &1 & 1& 1&1 &
 & \\
%2eme ligne
F(x) & \textbf{0} & 1& \textbf{1} & 0 &
 &0 &0& 0&0 & 0&
 &0 &\textbf{0} & 1&1 & &\\
%3eme ligne
 &1 & 1& 1& \textbf{1}&
 &0 &0 &0 &0 &0 &
& \textbf{0} & 1& \textbf{1} & \textbf{0} &
 & \\
% 4eme ligne
 &0 &\textbf{0} &0 &0 &
 &\textbf{1} &1 &0 &\textbf{1} &\textbf{1} &
 &1 &0 & 0&0 &
 &\\\hline
$x^{0}$ & & & & & $x^{4}$ & & & & & & $x^{9}$ & & & & & $x^{13}$ & \\
4 &0 &0 &4 &6&6 &7 &15 &7 &7 &7 &7&5  &1 &3 &1 &1 &  \\ & & & && & & & & & &  & & & & & & \\
%1ere ligne
0 & & & & &
0 & & $\xrightarrow{1} 1$ & $\xrightarrow{1} 0$ & & &
0 & & & & &
0 & \\
%2eme ligne
1 & $\xrightarrow{2} 0$ & & $\xrightarrow{2} 1$ &  &
1 & & & & & &
1 & & $\xrightarrow{2} 0$ & & & 0 &\\
%3eme ligne
0 & & & & $\xrightarrow{3} 1$ &
1 & & & & & &
1 & $\xrightarrow{3} 0$ & & $\xrightarrow{3} 1$ & $\xrightarrow{3} 0$ &
0 &\\
% 4eme ligne
0 & & $\xrightarrow{4} 0$ & & &
0 &$\xrightarrow{4} 1$ & & & $\xrightarrow{4} 1$&$\xrightarrow{4} 1$ &
1 & & & & &
1 &\\
\hline\hline
\end{tabular}\\
\vspace{0.5cm}
Binary Output: $x_1^{0}x_2^{0}x_3^{0}x_4^{0}x_5^{0}x_1^{4}x_2^{4}x_3^{4}x_4^{4}x_5^{4}x_1^{9}x_2^{9}x_3^{9}x_4^{9}x_5^{9}x_1^{13}x_2^{13}... = 0100011001110001...$

Integer Output:
$x^{0},x^{0},x^{4},x^{6},x^{8}... = 6,7,1...$
\caption{Application example}
\label{table application example}
\end{table*}
\end{tiny}
So, in this example, the generated binary digits are: 0100011001110001... Or the integers are: 6,7,1...




% \section{NIST statistical test suite}
% \subsection{Presentation}
% 
% Among the numerous standard tests for pseudo-randomness, a convincing way to prove the quality of the produced sequences is to confront them with the NIST (National Institute of Standards and Technology) Statistical Test Suite SP 800-22, 
% released by the Information Technology Laboratory in August 11, 2010.
% 
% The NIST test suite, SP 800-22, is a statistical package consisting of 15 tests. They were developed to measure the randomness of (arbitrarily long) binary sequences produced by either hardware or software based cryptographic pseudorandom number generators. These tests focus on a variety of different types of non-randomness that could occur in such sequences. These 15 tests include in the NIST test suite are described in \cite{ANDREW2008}.
% 
% 
% \subsection{Interpretation of empirical results}
% For all 15 tests, the significance level $\alpha$ was set to $1\%$. If a p-value is greater than 0.01, the keystream is accepted as random with a confidence of $99\%$; otherwise, it is considered as non-random.
% For each statistical test, a set of p-values is produced from a set of sequences obtained by our generator (i.e., 100 sequences are generated and tested, hence 100 p-values are produced). 
% 
% Empirical results can be interpreted in various ways. In this paper, 
% we check whether $\mathbb{P}_T$ (P-values of p-values), which arise via the application of a chi-square test, were all higher than 0.0001. This means
% that all p-values are uniformly distributed over (0, 1) interval as expected for an ideal random number generator. For further
% details on the NIST statistical test suite, the reader is referred to\cite{ANDREW2008}.
% 
% \subsection{NIST test suite results}  
% 
% Table~\ref{The passing rate} shows $\mathbb{P}_T$ of the sequences based on discrete chaotic iterations using different ``iteration'' functions. If there are at least two statistical values in a test, the test is marked with an asterisk and the average value is computed to characterize the statistical values. 
% 
% We can conclude from Table \ref{The passing rate} that 




% \clearpage
% \section*{ANNEXE}
% \begin{tiny}
% \newsavebox{\tablebox}
% \begin{lrbox}{\tablebox}
% % \caption{SP 800-22 test results ($\mathbb{P}_T$)}
% \renewcommand{\arraystretch}{1.3}
% 
% \label{The passing rate}
% \centering
%   \begin{tabular}{lccccccccccccccc}
%     \hline
% 
%   Mapping function&FT&FBT  &CST*&RT&LROBT&BMRT&DFTT&NOTMT*&OTMT&MUST&AET&RET*&REVT*&ST*&LCT  \\ \hline
% (14, 14, 12, 12, 10, 10, 9, 8, 6, 6, 4, 4, 2, 2, 0, 0)&0.000000	&  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.035374&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN&	  0.000000&	  0.025100	\\ \hline
% (14, 14, 12, 12, 10, 10, 9, 9, 6, 6, 4, 4, 2, 2, 1, 0)& 0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.699300&	  0.000000&	  0.020813&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN&	  0.000200&	  0.051900\\ \hline
% (14, 14, 12, 12, 11, 10, 9, 8, 6, 6, 4, 4, 2, 2, 1, 0)& 0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.657900&	  0.000000&	  0.007594&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN&	  0.000000&	  0.554400\\ \hline
% (14, 14, 12, 12, 11, 10, 9, 9, 6, 6, 4, 4, 2, 2, 1, 0)&0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.494300&	  0.000000&	  0.017793&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN&	  0.000000&	  0.595500	\\ \hline
% (14, 14, 12, 12, 11, 10, 9, 9, 6, 6, 4, 4, 2, 2, 1, 1)& 0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.514100&	  0.045600&	  0.000000&	  0.033795&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN&	  0.000000&	  0.514100\\ \hline
% (14, 14, 12, 12, 11, 10, 9, 9, 6, 6, 4, 4, 3, 2, 1, 0)&0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.779100&	  0.000000&	  0.022912&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN&	  0.076850&	  0.191600	\\ \hline
% (14, 14, 12, 12, 11, 11, 9, 9, 6, 6, 4, 4, 3, 2, 1, 1) &0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.275700&	  0.000000&	  0.040998&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN&	  0.191900&	  0.779100\\ \hline
% (14, 14, 13, 12, 11, 10, 9, 8, 6, 6, 4, 4, 2, 2, 1, 0) & 0.000000&	  0.000000&	  0.000000	&  0.000000&	  0.000000&	  0.595500&	  0.000000&	  0.029283&	  0.000000	&  0.000000	&  0.000000&	NaN&	NaN&	  0.000000&	  0.998800\\ \hline
% (14, 14, 13, 12, 11, 10, 9, 8, 6, 6, 4, 4, 3, 2, 1, 0) &0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.867600&	  0.000000&	  0.041652&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN&	  0.090750&	  0.202200	\\ \hline
% (14, 14, 13, 12, 11, 10, 9, 9, 6, 6, 4, 4, 2, 2, 1, 0) &0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.236800&	  0.000000&	  0.031913&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN&	  0.000000&	  0.779100\\ \hline
% (14, 14, 13, 12, 11, 10, 9, 9, 6, 6, 4, 4, 2, 2, 1, 1) &0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.897700&	  0.000000&	  0.062527&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN&	  0.000000&	  0.574900\\ \hline
% (14, 14, 13, 12, 11, 10, 9, 9, 6, 6, 4, 4, 3, 2, 1, 0) & 0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.883100&	  0.000000&	  0.026912&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN&	  0.000050&	  0.759700	\\ \hline
% (14, 14, 13, 12, 11, 10, 9, 9, 6, 6, 4, 4, 3, 2, 1, 1) &0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.739900&	  0.000100&	  0.042912&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN&	  0.152050&	  0.181500	\\ \hline
% (14, 14, 13, 12, 11, 10, 9, 9, 6, 6, 5, 4, 3, 2, 1, 0) & 0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.096500&	  0.595500	&  0.236800	&  0.088732&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN&	  0.441550&	  0.924000	\\ \hline
% (14, 14, 13, 12, 11, 11, 9, 9, 6, 6, 4, 4, 2, 2, 1, 1) & 0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.066800&	  0.000000&	  0.038274&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN	&  0.000000&	  0.181500	\\ \hline
% (14, 14, 13, 12, 11, 11, 9, 9, 6, 6, 4, 4, 3, 2, 1, 1) &0.978000&	  0.000000&	  0.372750&	  0.000000&	  0.000000&	  0.304100&	  0.000000&	  0.027336&	  0.000000&	  0.000000&	  0.000000&	  0.010887&	  0.544361&	  0.287450&	  0.834300\\ \hline
% (14, 14, 13, 12, 11, 11, 9, 9, 6, 6, 5, 4, 2, 2, 1, 0) & 0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.494300&	  0.616300&	  0.964200&	  0.060961&	  0.030800&	  0.000000&	  0.000000&	NaN&	NaN&	  0.000000&	  0.075700\\ \hline
% (14, 14, 13, 12, 11, 11, 9, 9, 6, 6, 5, 4, 2, 2, 1, 1) &0.657900&	  0.000000&	  0.594500&	  0.000000&	  0.000000&	  0.162600&	  0.000000&	  0.087611&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.512061&	  0.200550&	  0.798100\\ \hline
% (14, 14, 13, 12, 11, 11, 9, 9, 6, 6, 5, 4, 3, 2, 1, 0) &0.514100&	  0.006600&	  0.766800&	  0.000000	&  0.000000&	  0.739900&	  0.000000	&  0.072541&	  0.000000&	  0.000000&	  0.000000&	  0.209838&	  0.536178&	  0.048250&	  0.350400\\ \hline
% (15, 14, 13, 12, 11, 10, 9, 8, 6, 6, 5, 4, 3, 2, 1, 0) &0.000000&	  0.000000&	  0.000000&	  0.000000	&  0.045600&	  0.883100&	  0.000000&	  0.049661&	  0.000000&	  0.000000&	  0.000000&	NaN&	NaN&	  0.061150&	  0.924000	\\ \hline
% (15, 14, 13, 12, 11, 10, 9, 9, 6, 6, 5, 4, 3, 2, 1, 0)& 0.851300&	  0.162600&	  0.870250&	  0.000000&	  0.000000&	  0.678600&	  0.008200&	  0.084955&	  0.000000&	  0.000000&	  0.000000&	  0.283637&	  0.403839&	  0.379850&	  0.616300\\ \hline
% (8,8,9,9,10,10,11,11,4,4,5,5,6,6,7,7)&0.181500	&  0.000000	&  0.000000&	  0.000000	&  0.000000	&  0.366900&	  0.000000&	  0.000150&	  0.000000&	  0.000000&	  0.000000&	NaN&	  0.216889&	  0.000000&	  0.102500\\ \hline
% (8, 8, 8, 8, 8, 8, 8, 8, 7, 7, 7, 7, 7, 7, 7, 7)& 0.000100&	  0.000000&	  0.000000&	  0.000000&	  0.000000&	  0.574900&	  0.000000&	  0.006918&	  0.000000&	  0.000000&	  0.000000&	NaN&	  0.005761&	  0.000000&	  0.554400	\\ 
% 
% 
%     \hline
%   \end{tabular}
% 
% \end{lrbox}
% \rotatebox[origin=c]{90}{\usebox{\tablebox}}
% \end{tiny}



==> instantiating_old.tex <==


\subsection{Models of Instantiating}

\JFC{toutes les notions présentes dans ces conditions suffisantes devraient avoir été présentées au préalable}



It has been proven in~\cite{} the following result:

\begin{theorem}[Theorem III.6, p. 91 in~\cite{}]
\label{Th:Caractérisation   des   IC   chaotiques}  
Let  $f$ be a function from $\Bool^{n}$ to  $\Bool^{n}$. Then 
$G_f$ is chaotic  according to  Devaney if and only if  the graph
$\Gamma(f)$ is strongly connected.
\end{theorem}

Any function such that the graph $\Gamma(f)$ is strongly connected
is then a good candidate for being iterated as in the previous section and
then  for pseudo random number generating. 

Notice that the number of distinct iteration graphs is $2^n*2^n$ if $n$ is
the number of elements: first there are $2^n$ configuration;
next, each configuration may be linked to $n$ neighbors, 
leading to $2^n$ possibilities. 

For large number $n$ it is then not not tractable
first to generate all the graphs, and next to check 
the induced algorithms verify PRNG properties.


\JFC{Qian, please contribute here}
A first attempt is to consider small number $n$, for instance $n=2$. 
However, generated numbers in 
$\llbracket1 0, 3 \rrbracket$ are not sufficient to
exhaustively generate numbers  in $\llbracket1 0, 31 \rrbracket$
as confirmed in statistical test presented in figure~\ref{fig:neq2}.

\begin{figure}
\caption{Experiments wiht $n=2$}\label{fig:neq2}
\end{figure}


Let us focus on the second problem, i.e. the huge number of  
generated functions with potentially similar behavior due to the similarity of 
their graph. 
More formally, let us recall
the graph isomorphism definition.

\begin{definition}[Graph isomorphism]
Two directed graphs $G$ and $H$ are \emph{isomorphic} 
if there is a bijective mapping (permutation) $p$ from the vertices of $G$ to the vertices of $H$ such that
there is an arc from vertex $u$ to vertex  $v$  in $G$ 
if and only 
there is an arc from vertex $p(u)$ to vertex  $p(v)$  in $H$.
\end{definition}


Let $f$ be a function, $G$ be its iteration graph and $p$ 
be a permutation of vertices of $G$. 
Since $p(G)$ and $G$ are isomorphic,   
then iterating  $f$ 
(\textit{i.e.} traversing $G$) from the initial configuration $c$
amounts to iterating the function whose iteration graph is $p(G)$
from the configuration $p(c)$.
Graph isomorphism being an equivalence relation, the sequel only 
consider the quotient set of functions with this relation over their graph.
In other words, two functions are distinct if and only if their iteration
graph are not isomorphic.

In what follows, we the only focus on non isomorphic graphs of iterations
We then first recall a theorem that establish sufficient conditions
for strictly connected graphs.






\begin{theorem}[Theorem I,\cite{}]
\label{th:carac JFC}
If a map $f$ verifies the following conditions:
\begin{enumerate}
\item \label{cond:pp} the interaction graph $G(f)$ has no positive circuit; 
\item \label{cond:rl} each vertex of $G(f)$ is reachable from at least one 
vertex with a loop;
\item \label{cond:pn} for each pair $(i,j)$ in $\llbracket1;n\rrbracket^2$,   
  there is only one arc from $i$ to $j$, at most;
\end{enumerate} 
then the graph of iterations $\Gamma(f)$ is strongly connected.
\end{theorem}

Next section presents an direct application of this theorem.

\subsection{Generation example}
In this section, we consider that there are $n=3$ elements. 
As  instance of conditions \ref{cond:pp}.- \ref{cond:pn} we consider
the interaction graph $G(f)$ of $f$ given in figure~\ref{fig:interactiongraph}.

\begin{figure}
\begin{center}
%\includegraphics[width=3cm]{iteractionGraphExample.ps}
\includegraphics[width=3cm]{iteractionGraphExample.pdf}
\end{center}
\caption{Interaction Graph $G(f)$ of PRNG iteration function candidate}
\label{fig:interactiongraph}
\end{figure}



For each element $i$, it is not hard to compute the list images $f_i$ that 
are compliant with the interaction graph $G(f)$ and then to deduce
the function as the product of computed $f_i$.

We then have 
$f_0,f_1,f_2: \Bool^{n} \rightarrow \Bool$
with $f_0(x_0,\_,\_)= \overline{x_0}$.
For $f_1$, we have two candidates that are 
$f_{1a}(x_0,x_1,\_)= \overline{x_0}.\overline{x_1}$ or  
$f_{1b}(x_0,x_1,\_)= \overline{x_0}+\overline{x_1}$.
Finally for $f_2$, we have two candidates too that are 
$f_{2a}(x_0,x_1,\_)= x_0.\overline{x_1}$ or  
$f_{2b}(x_0,x_1,\_)= x_0+\overline{x_1}$.
The figure~\ref{fig:fs} gives the GTPIC of the four maps detailed above.



\begin{figure}
\centering
\subfigure[$(f_0,f_{1a},f_{2a})$]{
%\includegraphics[width=2cm]{iter_f0.ps}
\includegraphics[width=2cm]{iter_f0.pdf}}
%\label{fig:fs1}}
$\qquad\qquad$
\subfigure[$(f_0,f_{1a},f_{2b})$]{
%\includegraphics[width=2cm]{iter_f1.ps}
\includegraphics[width=2cm]{iter_f1.pdf}}
%\label{fig:fs2}}
$\qquad\qquad$
\subfigure[$(f_0,f_{1b},f_{2a})$]{
%\includegraphics[width=2cm]{iter_f2.ps}
\includegraphics[width=2cm]{iter_f2.pdf}}
%\label{fig:fs3}}
$\qquad\qquad$
\subfigure[$(f_0,f_{1b},f_{2b})$]{
%\includegraphics[width=2cm]{iter_f3.ps}
\includegraphics[width=2cm]{iter_f3.pdf}}
%\label{fig:fs4}}
\caption{GTPIC of Candidate Functions.} \label{fig:fs}
\end{figure}

\subsection{Generation Method}


% For $n$
% \item \label{cond:rl} each vertex of $G(f)$ is reachable from at least one 
% vertex with a loop;






